Reinforcement Learning from Automatic Feedback for High-Quality Unit Test Generation

Software testing is a crucial aspect of software development, and the creation of high-quality tests that adhere to best practices is essential for effective maintenance. Recently, Large Language Models (LLMs) have gained popularity for code generation, including the automated creation of test cases. However, these LLMs are often trained on vast amounts of publicly available code, which may include test cases that do not adhere to best practices and may even contain test smells (anti-patterns). To address this issue, we propose a novel technique called Reinforcement Learning from Static Quality Metrics (RLSQM). To begin, we analyze the anti-patterns generated by the LLM and show that LLMs can generate undesirable test smells. Thus, we train specific reward models for each static quality metric, then utilize Proximal Policy Optimization (PPO) to train models for optimizing a single quality metric at a time. Furthermore, we amalgamate these rewards into a unified reward model aimed at capturing different best practices and quality aspects of tests. By comparing RL-trained models with those trained using supervised learning, we provide insights into how reliably utilize RL to improve test generation quality and into the effects of various training strategies. Our experimental results demonstrate that the RL-optimized model consistently generated high-quality test cases compared to the base LLM, improving the model by up to 21%, and successfully generates nearly 100% syntactically correct code. RLSQM also outperformed GPT-4 on four out of seven metrics. This represents a significant step towards enhancing the overall efficiency and reliability of software testing through Reinforcement Learning and static quality metrics. Our data are available at https://figshare.com/s/ded476c8d4c221222849.

==> figures/additive-reward-old-v0.tex <==
% BEGIN TEX AUTOGENERATED BY create_rq3_plot.ipynb
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\goodmark{} \textbf{Best Practices}} & \multicolumn{2}{c}{\badmark{} \textbf{Test Smells}} \\ \cmidrule(rl){2-3} \cmidrule(l){4-5}
\textbf{Model} & Assertion & Focal call & \makecell[c]{Duplicate\\assert} & \makecell[c]{Conditional/\\Exception} \\
\midrule
Individual Reward & 92.8\% & 90.9\% & 1.35\% & 0.16\% \\
\midrule \goodmark{} Assertion + \goodmark{} Focal call & \colorbox{yellow!50}{\makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}}} & \colorbox{yellow!50}{\makecell[c]{88.4\% \\ \textcolor{black!20!red}{-2.5\%}}} & \makecell[c]{1.6\% \\ \textcolor{black!20!red}{+0.25\%}} & \makecell[c]{0.19\% \\ \textcolor{black!20!red}{+0.03\%}} \\
\goodmark{} Assertion + \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \colorbox{yellow!50}{\makecell[c]{94.8\% \\ \textcolor{black!30!green}{+2.0\%}}} & \makecell[c]{91.3\% \\ \textcolor{black!30!green}{+0.4\%}} & \colorbox{yellow!50}{\makecell[c]{1.78\% \\ \textcolor{black!20!red}{+0.43\%}}} & \makecell[c]{0.11\% \\ \textcolor{black!30!green}{-0.05\%}} \\
\goodmark{} Assertion + \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \colorbox{yellow!50}{\makecell[c]{96.8\% \\ \textcolor{black!30!green}{+4.0\%}}} & \makecell[c]{91.5\% \\ \textcolor{black!30!green}{+0.6\%}} & \makecell[c]{1.22\% \\ \textcolor{black!30!green}{-0.13\%}} & \colorbox{yellow!50}{\makecell[c]{0.06\% \\ \textcolor{black!30!green}{-0.1\%}}} \\
\goodmark{} Focal call + \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \makecell[c]{96.4\% \\ \textcolor{black!30!green}{+3.6\%}} & \colorbox{yellow!50}{\makecell[c]{90.5\% \\ \textcolor{black!20!red}{-0.4\%}}} & \colorbox{yellow!50}{\makecell[c]{1.46\% \\ \textcolor{black!20!red}{+0.11\%}}} & \makecell[c]{0.2\% \\ \textcolor{black!20!red}{+0.04\%}} \\
\goodmark{} Focal call + \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{96.5\% \\ \textcolor{black!30!green}{+3.7\%}} & \colorbox{yellow!50}{\makecell[c]{90.8\% \\ \textcolor{black!20!red}{-0.1\%}}} & \makecell[c]{0.55\% \\ \textcolor{black!30!green}{-0.8\%}} & \colorbox{yellow!50}{\makecell[c]{0.03\% \\ \textcolor{black!30!green}{-0.13\%}}} \\
\makecell[l]{\badmark{} Duplicate\\\quad{}assert} \hspace{-6em} + \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}} & \makecell[c]{87.9\% \\ \textcolor{black!20!red}{-3.0\%}} & \colorbox{yellow!50}{\makecell[c]{1.98\% \\ \textcolor{black!20!red}{+0.63\%}}} & \colorbox{yellow!50}{\makecell[c]{0.15\% \\ \textcolor{black!30!green}{-0.01\%}}} \\
\midrule \goodmark{} Assertion + \goodmark{} Focal call + \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \colorbox{yellow!50}{\makecell[c]{95.3\% \\ \textcolor{black!30!green}{+2.5\%}}} & \colorbox{yellow!50}{\makecell[c]{90.0\% \\ \textcolor{black!20!red}{-0.9\%}}} & \colorbox{yellow!50}{\makecell[c]{1.73\% \\ \textcolor{black!20!red}{+0.38\%}}} & \makecell[c]{0.13\% \\ \textcolor{black!30!green}{-0.03\%}} \\
\goodmark{} Assertion + \goodmark{} Focal call + \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \colorbox{yellow!50}{\makecell[c]{88.0\% \\ \textcolor{black!20!red}{-4.8\%}}} & \colorbox{yellow!50}{\makecell[c]{76.1\% \\ \textcolor{black!20!red}{-14.8\%}}} & \makecell[c]{0.78\% \\ \textcolor{black!30!green}{-0.57\%}} & \colorbox{yellow!50}{\makecell[c]{0.42\% \\ \textcolor{black!20!red}{+0.26\%}}} \\
\goodmark{} Focal call + \makecell[l]{\badmark{} Duplicate\\\quad{}assert} + \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{92.9\% \\ \textcolor{black!30!green}{+0.1\%}} & \colorbox{yellow!50}{\makecell[c]{92.8\% \\ \textcolor{black!30!green}{+1.9\%}}} & \colorbox{yellow!50}{\makecell[c]{0.85\% \\ \textcolor{black!30!green}{-0.5\%}}} & \colorbox{yellow!50}{\makecell[c]{0.08\% \\ \textcolor{black!30!green}{-0.08\%}}} \\
\midrule All 4 properties & \makecell[c]{89.8\% \\ \textcolor{black!20!red}{-3.0\%}} & \makecell[c]{84.7\% \\ \textcolor{black!20!red}{-6.2\%}} & \makecell[c]{1.19\% \\ \textcolor{black!30!green}{-0.16\%}} & \makecell[c]{0.21\% \\ \textcolor{black!20!red}{+0.05\%}} \\
\bottomrule
\end{tabular}
% END TEX AUTOGENERATED BY create_rq3_plot.ipynb

==> figures/additive-reward-v1.tex <==





% BEGIN TEX AUTOGENERATED BY create_rq3_plot.ipynb
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{\goodmark{} Best Practices}} & \multicolumn{2}{c}{\textbf{\badmark{} Test Smells}} \\ \cmidrule(rl){2-3} \cmidrule(l){4-5}
\textbf{Model} & Assert & Focal & \makecell[c]{Dupl.\\Assert} & \makecell[c]{Cond./\\Exc.} \\
\midrule
Best Individual Reward & 92.8\% & 90.9\% & 1.35\% & 0.16\% \\
\midrule Assert + Focal & \colorbox{yellow!50}{\makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}}} & \colorbox{yellow!50}{\makecell[c]{88.4\% \\ \textcolor{black!20!red}{-2.5\%}}} & \makecell[c]{1.6\% \\ \textcolor{black!20!red}{+0.25\%}} & \makecell[c]{0.19\% \\ \textcolor{black!20!red}{+0.03\%}} \\
Assert + \makecell[l]{DA} & \colorbox{yellow!50}{\makecell[c]{94.8\% \\ \textcolor{black!30!green}{+2.0\%}}} & \makecell[c]{91.3\% \\ \textcolor{black!30!green}{+0.4\%}} & \colorbox{yellow!50}{\makecell[c]{1.78\% \\ \textcolor{black!20!red}{+0.43\%}}} & \makecell[c]{0.11\% \\ \textcolor{black!30!green}{-0.05\%}} \\
Assert + \makecell[l]{CEH} & \colorbox{yellow!50}{\makecell[c]{96.8\% \\ \textcolor{black!30!green}{+4.0\%}}} & \makecell[c]{91.5\% \\ \textcolor{black!30!green}{+0.6\%}} & \makecell[c]{1.22\% \\ \textcolor{black!30!green}{-0.13\%}} & \colorbox{yellow!50}{\makecell[c]{0.06\% \\ \textcolor{black!30!green}{-0.1\%}}} \\
Focal + \makecell[l]{DA} & \makecell[c]{96.4\% \\ \textcolor{black!30!green}{+3.6\%}} & \colorbox{yellow!50}{\makecell[c]{90.5\% \\ \textcolor{black!20!red}{-0.4\%}}} & \colorbox{yellow!50}{\makecell[c]{1.46\% \\ \textcolor{black!20!red}{+0.11\%}}} & \makecell[c]{0.2\% \\ \textcolor{black!20!red}{+0.04\%}} \\
Focal + \makecell[l]{CEH} & \makecell[c]{96.5\% \\ \textcolor{black!30!green}{+3.7\%}} & \colorbox{yellow!50}{\makecell[c]{90.8\% \\ \textcolor{black!20!red}{-0.1\%}}} & \makecell[c]{0.55\% \\ \textcolor{black!30!green}{-0.8\%}} & \colorbox{yellow!50}{\makecell[c]{0.03\% \\ \textcolor{black!30!green}{-0.13\%}}} \\
DA + \makecell[l]{CEH} & \makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}} & \makecell[c]{87.9\% \\ \textcolor{black!20!red}{-3.0\%}} & \colorbox{yellow!50}{\makecell[c]{1.98\% \\ \textcolor{black!20!red}{+0.63\%}}} & \colorbox{yellow!50}{\makecell[c]{0.15\% \\ \textcolor{black!30!green}{-0.01\%}}} \\
\midrule Assert + Focal + DA & \colorbox{yellow!50}{\makecell[c]{95.3\% \\ \textcolor{black!30!green}{+2.5\%}}} & \colorbox{yellow!50}{\makecell[c]{90.0\% \\ \textcolor{black!20!red}{-0.9\%}}} & \colorbox{yellow!50}{\makecell[c]{1.73\% \\ \textcolor{black!20!red}{+0.38\%}}} & \makecell[c]{0.13\% \\ \textcolor{black!30!green}{-0.03\%}} \\
Assert + Focal + CEH & \colorbox{yellow!50}{\makecell[c]{88.0\% \\ \textcolor{black!20!red}{-4.8\%}}} & \colorbox{yellow!50}{\makecell[c]{76.1\% \\ \textcolor{black!20!red}{-14.8\%}}} & \makecell[c]{0.78\% \\ \textcolor{black!30!green}{-0.57\%}} & \colorbox{yellow!50}{\makecell[c]{0.42\% \\ \textcolor{black!20!red}{+0.26\%}}} \\
Focal + DA + CEH & \makecell[c]{92.9\% \\ \textcolor{black!30!green}{+0.1\%}} & \colorbox{yellow!50}{\makecell[c]{92.8\% \\ \textcolor{black!30!green}{+1.9\%}}} & \colorbox{yellow!50}{\makecell[c]{0.85\% \\ \textcolor{black!30!green}{-0.5\%}}} & \colorbox{yellow!50}{\makecell[c]{0.08\% \\ \textcolor{black!30!green}{-0.08\%}}} \\
\midrule All 4 properties & \makecell[c]{89.8\% \\ \textcolor{black!20!red}{-3.0\%}} & \makecell[c]{84.7\% \\ \textcolor{black!20!red}{-6.2\%}} & \makecell[c]{1.19\% \\ \textcolor{black!30!green}{-0.16\%}} & \makecell[c]{0.21\% \\ \textcolor{black!20!red}{+0.05\%}} \\
\bottomrule
\end{tabular}
% END TEX AUTOGENERATED BY create_rq3_plot.ipynb

==> figures/individual-rewards.tex <==
% BEGIN TEX AUTOGENERATED BY create_rq2_plot.ipynb
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{3}{c}{\goodmark{} \textbf{Necessary/Best Practices}} & \multicolumn{2}{c}{\goodmark{} \textbf{Documentation}} & \multicolumn{2}{c}{\badmark{} \textbf{Test Smells}} \\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-8}
\textbf{Model} & \makecell[c]{Syntax\\Correct} & Assert & Focal call & Descr. & Comment & \makecell[c]{Duplicate\\assert} & \makecell[c]{Conditional/\\Exception} \\
\midrule
GPT-4 & 90.9\% & 81.2\% & 90.5\% & 23.1\% & 77.6\% & 0.56\% & 2.51\% \\
\midrule Base & 86.6\% & 73.4\% & 72.9\% & 10.7\% & 19.5\% & 2.77\% & 2.56\% \\
\midrule SFT & 88.4\% & 84.9\% & 80.0\% & 5.2\% & 15.3\% & 1.49\% & 0.23\% \\
\midrule
\goodmark{} Assertion & \makecell[c]{99.4\% \\ \textcolor{black!30!green}{+11.0\%}} & \colorbox{yellow!50}{\makecell[c]{92.8\% \\ \textcolor{black!30!green}{+7.9\%}}} & \makecell[c]{91.4\% \\ \textcolor{black!30!green}{+11.4\%}} & \makecell[c]{10.3\% \\ \textcolor{black!30!green}{+5.1\%}} & \makecell[c]{5.5\% \\ \textcolor{black!20!red}{-9.8\%}} & \makecell[c]{1.22\% \\ \textcolor{black!30!green}{-0.27\%}} & \makecell[c]{0.16\% \\ \textcolor{black!30!green}{-0.07\%}} \\
\goodmark{} Focal call & \makecell[c]{98.8\% \\ \textcolor{black!30!green}{+10.4\%}} & \makecell[c]{95.2\% \\ \textcolor{black!30!green}{+10.3\%}} & \colorbox{yellow!50}{\makecell[c]{90.9\% \\ \textcolor{black!30!green}{+10.9\%}}} & \makecell[c]{4.4\% \\ \textcolor{black!20!red}{-0.8\%}} & \makecell[c]{6.6\% \\ \textcolor{black!20!red}{-8.7\%}} & \makecell[c]{1.29\% \\ \textcolor{black!30!green}{-0.2\%}} & \makecell[c]{0.29\% \\ \textcolor{black!20!red}{+0.06\%}} \\
\midrule
\goodmark{} Descriptive & \makecell[c]{99.5\% \\ \textcolor{black!30!green}{+11.1\%}} & \makecell[c]{95.8\% \\ \textcolor{black!30!green}{+10.9\%}} & \makecell[c]{89.7\% \\ \textcolor{black!30!green}{+9.7\%}} & \colorbox{yellow!50}{\makecell[c]{3.6\% \\ \textcolor{black!20!red}{-1.6\%}}} & \makecell[c]{3.3\% \\ \textcolor{black!20!red}{-12.0\%}} & \makecell[c]{1.28\% \\ \textcolor{black!30!green}{-0.21\%}} & \makecell[c]{0.14\% \\ \textcolor{black!30!green}{-0.09\%}} \\
\goodmark{} Comment & \makecell[c]{99.1\% \\ \textcolor{black!30!green}{+10.7\%}} & \makecell[c]{94.4\% \\ \textcolor{black!30!green}{+9.5\%}} & \makecell[c]{92.8\% \\ \textcolor{black!30!green}{+12.8\%}} & \makecell[c]{4.1\% \\ \textcolor{black!20!red}{-1.1\%}} & \colorbox{yellow!50}{\makecell[c]{5.2\% \\ \textcolor{black!20!red}{-10.1\%}}} & \makecell[c]{1.58\% \\ \textcolor{black!20!red}{+0.09\%}} & \makecell[c]{0.14\% \\ \textcolor{black!30!green}{-0.09\%}} \\
\midrule
\makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \makecell[c]{99.0\% \\ \textcolor{black!30!green}{+10.6\%}} & \makecell[c]{94.8\% \\ \textcolor{black!30!green}{+9.9\%}} & \makecell[c]{91.7\% \\ \textcolor{black!30!green}{+11.7\%}} & \makecell[c]{3.1\% \\ \textcolor{black!20!red}{-2.1\%}} & \makecell[c]{7.3\% \\ \textcolor{black!20!red}{-8.0\%}} & \colorbox{yellow!50}{\makecell[c]{1.35\% \\ \textcolor{black!30!green}{-0.14\%}}} & \makecell[c]{0.12\% \\ \textcolor{black!30!green}{-0.11\%}} \\
\makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{97.0\% \\ \textcolor{black!30!green}{+8.6\%}} & \makecell[c]{92.7\% \\ \textcolor{black!30!green}{+7.8\%}} & \makecell[c]{84.8\% \\ \textcolor{black!30!green}{+4.8\%}} & \makecell[c]{4.6\% \\ \textcolor{black!20!red}{-0.6\%}} & \makecell[c]{9.4\% \\ \textcolor{black!20!red}{-5.9\%}} & \makecell[c]{1.07\% \\ \textcolor{black!30!green}{-0.42\%}} & \colorbox{yellow!50}{\makecell[c]{0.16\% \\ \textcolor{black!30!green}{-0.07\%}}} \\
\bottomrule
\end{tabular}
% END TEX AUTOGENERATED BY create_rq2_plot.ipynb

==> figures/iterative-reward-old-v0.tex <==
% BEGIN TEX AUTOGENERATED BY create_rq3_plot_iterative.ipynb
\begin{tabular}{lclcccccc}
\toprule
& & & \multicolumn{2}{c}{\goodmark{} \textbf{Best Practices}} & \multicolumn{2}{c}{\badmark{} \textbf{Test Smells}} \\ \cmidrule(rl){4-5} \cmidrule(l){6-7}
\textbf{\nth{1} stage} & & \textbf{\nth{2} stage} & Assertion & Focal call & \makecell[c]{Duplicate\\assert} & \makecell[c]{Conditional/\\Exception} \\
\midrule
\multicolumn{3}{l}{Best Individual Reward} & 92.8\% & 90.9\% & 1.35\% & 0.16\% \\
\midrule
\goodmark{} Assertion & $\rightarrow$ & \goodmark{} Focal call & \colorbox{yellow!50}{\makecell[c]{93.5\% \\ \textcolor{black!30!green}{+0.7\%}}} & \colorbox{orange!50}{\makecell[c]{89.9\% \\ \textcolor{black!20!red}{-1.0\%}}} & \makecell[c]{1.42\% \\ \textcolor{black!20!red}{+0.07\%}} & \makecell[c]{0.12\% \\ \textcolor{black!30!green}{-0.04\%}} \\
\goodmark{} Assertion & $\rightarrow$ & \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \colorbox{yellow!50}{\makecell[c]{95.9\% \\ \textcolor{black!30!green}{+3.1\%}}} & \makecell[c]{88.3\% \\ \textcolor{black!20!red}{-2.6\%}} & \colorbox{orange!50}{\makecell[c]{1.44\% \\ \textcolor{black!20!red}{+0.09\%}}} & \makecell[c]{0.09\% \\ \textcolor{black!30!green}{-0.07\%}} \\
\goodmark{} Assertion & $\rightarrow$ & \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \colorbox{yellow!50}{\makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}}} & \makecell[c]{91.6\% \\ \textcolor{black!30!green}{+0.7\%}} & \makecell[c]{0.76\% \\ \textcolor{black!30!green}{-0.59\%}} & \colorbox{orange!50}{\makecell[c]{0.39\% \\ \textcolor{black!20!red}{+0.23\%}}} \\
\midrule
\goodmark{} Focal call & $\rightarrow$ & \goodmark{} Assertion & \colorbox{orange!50}{\makecell[c]{96.7\% \\ \textcolor{black!30!green}{+3.9\%}}} & \colorbox{yellow!50}{\makecell[c]{90.7\% \\ \textcolor{black!20!red}{-0.2\%}}} & \makecell[c]{2.08\% \\ \textcolor{black!20!red}{+0.73\%}} & \makecell[c]{0.31\% \\ \textcolor{black!20!red}{+0.15\%}} \\
\goodmark{} Focal call & $\rightarrow$ & \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \makecell[c]{98.1\% \\ \textcolor{black!30!green}{+5.3\%}} & \colorbox{yellow!50}{\makecell[c]{91.3\% \\ \textcolor{black!30!green}{+0.4\%}}} & \colorbox{orange!50}{\makecell[c]{1.29\% \\ \textcolor{black!30!green}{-0.06\%}}} & \makecell[c]{0.27\% \\ \textcolor{black!20!red}{+0.11\%}} \\
\goodmark{} Focal call & $\rightarrow$ & \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{96.4\% \\ \textcolor{black!30!green}{+3.6\%}} & \colorbox{yellow!50}{\makecell[c]{93.4\% \\ \textcolor{black!30!green}{+2.5\%}}} & \makecell[c]{0.94\% \\ \textcolor{black!30!green}{-0.41\%}} & \colorbox{orange!50}{\makecell[c]{0.16\% \\ \textcolor{black!30!green}{+0.0\%}}} \\
\midrule
\makecell[l]{\badmark{} Duplicate\\\quad{}assert} & $\rightarrow$ & \goodmark{} Assertion & \colorbox{orange!50}{\makecell[c]{97.4\% \\ \textcolor{black!30!green}{+4.6\%}}} & \makecell[c]{90.4\% \\ \textcolor{black!20!red}{-0.5\%}} & \colorbox{yellow!50}{\makecell[c]{2.78\% \\ \textcolor{black!20!red}{+1.43\%}}} & \makecell[c]{0.29\% \\ \textcolor{black!20!red}{+0.13\%}} \\
\makecell[l]{\badmark{} Duplicate\\\quad{}assert} & $\rightarrow$ & \goodmark{} Focal call & \makecell[c]{95.3\% \\ \textcolor{black!30!green}{+2.5\%}} & \colorbox{orange!50}{\makecell[c]{87.8\% \\ \textcolor{black!20!red}{-3.1\%}}} & \colorbox{yellow!50}{\makecell[c]{2.41\% \\ \textcolor{black!20!red}{+1.06\%}}} & \makecell[c]{0.25\% \\ \textcolor{black!20!red}{+0.09\%}} \\
\makecell[l]{\badmark{} Duplicate\\\quad{}assert} & $\rightarrow$ & \makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & \makecell[c]{94.5\% \\ \textcolor{black!30!green}{+1.7\%}} & \makecell[c]{89.9\% \\ \textcolor{black!20!red}{-1.0\%}} & \colorbox{yellow!50}{\makecell[c]{2.4\% \\ \textcolor{black!20!red}{+1.05\%}}} & \colorbox{orange!50}{\makecell[c]{0.22\% \\ \textcolor{black!20!red}{+0.06\%}}} \\
\midrule
\makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & $\rightarrow$ & \goodmark{} Assertion & \colorbox{orange!50}{\makecell[c]{95.8\% \\ \textcolor{black!30!green}{+3.0\%}}} & \makecell[c]{85.6\% \\ \textcolor{black!20!red}{-5.3\%}} & \makecell[c]{1.36\% \\ \textcolor{black!20!red}{+0.01\%}} & \colorbox{yellow!50}{\makecell[c]{0.32\% \\ \textcolor{black!20!red}{+0.16\%}}} \\
\makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & $\rightarrow$ & \goodmark{} Focal call & \makecell[c]{96.1\% \\ \textcolor{black!30!green}{+3.3\%}} & \colorbox{orange!50}{\makecell[c]{86.0\% \\ \textcolor{black!20!red}{-4.9\%}}} & \makecell[c]{3.06\% \\ \textcolor{black!20!red}{+1.71\%}} & \colorbox{yellow!50}{\makecell[c]{0.12\% \\ \textcolor{black!30!green}{-0.04\%}}} \\
\makecell[l]{\badmark{} Conditional/\\\quad{}Exception} & $\rightarrow$ & \makecell[l]{\badmark{} Duplicate\\\quad{}assert} & \makecell[c]{88.7\% \\ \textcolor{black!20!red}{-4.1\%}} & \makecell[c]{80.2\% \\ \textcolor{black!20!red}{-10.7\%}} & \colorbox{orange!50}{\makecell[c]{1.17\% \\ \textcolor{black!30!green}{-0.18\%}}} & \colorbox{yellow!50}{\makecell[c]{0.11\% \\ \textcolor{black!30!green}{-0.05\%}}} \\
\bottomrule
\end{tabular}
% END TEX AUTOGENERATED BY create_rq3_plot_iterative.ipynb

==> figures/iterative-reward-v1.tex <==
% BEGIN TEX AUTOGENERATED BY create_rq3_plot_iterative.ipynb
\begin{tabular}{llcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{\goodmark{} Best Practices}} & \multicolumn{2}{c}{\textbf{\badmark{} Test Smells}} \\ \cmidrule(rl){2-3} \cmidrule(l){4-5}
\textbf{\nth{1} stage $\rightarrow$ \nth{2} stage} & Assert & Focal & \makecell[l]{Dupl.\\Assert} & \makecell[l]{Cond./\\Exc.} \\
\midrule
\multicolumn{1}{l}{Best Individual Reward} & 92.8\% & 90.9\% & 1.35\% & 0.16\% \\
\midrule
Assert $\rightarrow$ Focal & \colorbox{yellow!50}{\makecell[c]{93.5\% \\ \textcolor{black!30!green}{+0.7\%}}} & \colorbox{orange!50}{\makecell[c]{89.9\% \\ \textcolor{black!20!red}{-1.0\%}}} & \makecell[c]{1.42\% \\ \textcolor{black!20!red}{+0.07\%}} & \makecell[c]{0.12\% \\ \textcolor{black!30!green}{-0.04\%}} \\
Assert $\rightarrow$ \makecell[l]{DA} & \colorbox{yellow!50}{\makecell[c]{95.9\% \\ \textcolor{black!30!green}{+3.1\%}}} & \makecell[c]{88.3\% \\ \textcolor{black!20!red}{-2.6\%}} & \colorbox{orange!50}{\makecell[c]{1.44\% \\ \textcolor{black!20!red}{+0.09\%}}} & \makecell[c]{0.09\% \\ \textcolor{black!30!green}{-0.07\%}} \\
Assert $\rightarrow$ \makecell[l]{CEH} & \colorbox{yellow!50}{\makecell[c]{93.1\% \\ \textcolor{black!30!green}{+0.3\%}}} & \makecell[c]{91.6\% \\ \textcolor{black!30!green}{+0.7\%}} & \makecell[c]{0.76\% \\ \textcolor{black!30!green}{-0.59\%}} & \colorbox{orange!50}{\makecell[c]{0.39\% \\ \textcolor{black!20!red}{+0.23\%}}} \\
\midrule
Focal $\rightarrow$ Assert & \colorbox{orange!50}{\makecell[c]{96.7\% \\ \textcolor{black!30!green}{+3.9\%}}} & \colorbox{yellow!50}{\makecell[c]{90.7\% \\ \textcolor{black!20!red}{-0.2\%}}} & \makecell[c]{2.08\% \\ \textcolor{black!20!red}{+0.73\%}} & \makecell[c]{0.31\% \\ \textcolor{black!20!red}{+0.15\%}} \\
Focal $\rightarrow$ \makecell[l]{DA} & \makecell[c]{98.1\% \\ \textcolor{black!30!green}{+5.3\%}} & \colorbox{yellow!50}{\makecell[c]{91.3\% \\ \textcolor{black!30!green}{+0.4\%}}} & \colorbox{orange!50}{\makecell[c]{1.29\% \\ \textcolor{black!30!green}{-0.06\%}}} & \makecell[c]{0.27\% \\ \textcolor{black!20!red}{+0.11\%}} \\
Focal $\rightarrow$ \makecell[l]{CEH} & \makecell[c]{96.4\% \\ \textcolor{black!30!green}{+3.6\%}} & \colorbox{yellow!50}{\makecell[c]{93.4\% \\ \textcolor{black!30!green}{+2.5\%}}} & \makecell[c]{0.94\% \\ \textcolor{black!30!green}{-0.41\%}} & \colorbox{orange!50}{\makecell[c]{0.16\% \\ \textcolor{black!30!green}{+0.0\%}}} \\
\midrule
DA $\rightarrow$ Assert & \colorbox{orange!50}{\makecell[c]{97.4\% \\ \textcolor{black!30!green}{+4.6\%}}} & \makecell[c]{90.4\% \\ \textcolor{black!20!red}{-0.5\%}} & \colorbox{yellow!50}{\makecell[c]{2.78\% \\ \textcolor{black!20!red}{+1.43\%}}} & \makecell[c]{0.29\% \\ \textcolor{black!20!red}{+0.13\%}} \\
DA $\rightarrow$ Focal & \makecell[c]{95.3\% \\ \textcolor{black!30!green}{+2.5\%}} & \colorbox{orange!50}{\makecell[c]{87.8\% \\ \textcolor{black!20!red}{-3.1\%}}} & \colorbox{yellow!50}{\makecell[c]{2.41\% \\ \textcolor{black!20!red}{+1.06\%}}} & \makecell[c]{0.25\% \\ \textcolor{black!20!red}{+0.09\%}} \\
DA $\rightarrow$ \makecell[l]{CEH} & \makecell[c]{94.5\% \\ \textcolor{black!30!green}{+1.7\%}} & \makecell[c]{89.9\% \\ \textcolor{black!20!red}{-1.0\%}} & \colorbox{yellow!50}{\makecell[c]{2.4\% \\ \textcolor{black!20!red}{+1.05\%}}} & \colorbox{orange!50}{\makecell[c]{0.22\% \\ \textcolor{black!20!red}{+0.06\%}}} \\
\midrule
CEH $\rightarrow$ Assert & \colorbox{orange!50}{\makecell[c]{95.8\% \\ \textcolor{black!30!green}{+3.0\%}}} & \makecell[c]{85.6\% \\ \textcolor{black!20!red}{-5.3\%}} & \makecell[c]{1.36\% \\ \textcolor{black!20!red}{+0.01\%}} & \colorbox{yellow!50}{\makecell[c]{0.32\% \\ \textcolor{black!20!red}{+0.16\%}}} \\
CEH $\rightarrow$ Focal & \makecell[c]{96.1\% \\ \textcolor{black!30!green}{+3.3\%}} & \colorbox{orange!50}{\makecell[c]{86.0\% \\ \textcolor{black!20!red}{-4.9\%}}} & \makecell[c]{3.06\% \\ \textcolor{black!20!red}{+1.71\%}} & \colorbox{yellow!50}{\makecell[c]{0.12\% \\ \textcolor{black!30!green}{-0.04\%}}} \\
CEH $\rightarrow$ \makecell[l]{DA} & \makecell[c]{88.7\% \\ \textcolor{black!20!red}{-4.1\%}} & \makecell[c]{80.2\% \\ \textcolor{black!20!red}{-10.7\%}} & \colorbox{orange!50}{\makecell[c]{1.17\% \\ \textcolor{black!30!green}{-0.18\%}}} & \colorbox{yellow!50}{\makecell[c]{0.11\% \\ \textcolor{black!30!green}{-0.05\%}}} \\
\bottomrule
\end{tabular}
% END TEX AUTOGENERATED BY create_rq3_plot_iterative.ipynb

==> figures/sft-rl-parameters.tex <==
\begin{table}[t]
    \centering
    \caption{Parameters used for supervised fine-tuning (left) and RL fine-tuning (right). \BENJAMIN{Consider moving to data package.}
    % \BENJAMIN{TODO: Reference in the text for SFT and RL.}
    }
    \label{tab:training-parameters}
    % 
    \begin{tabular}[t]{lr}
    \toprule
    \textbf{Parameter} & \textbf{Value} \\
    \midrule
    Epochs & 5 \\
    Batch size & 178 (0.2\% data) \\
    % \makecell[l]{Learning rate\\
    % \hspace{1cm}LR schedule\\
    % \hspace{1cm}LR warmup steps
    % } & \xxx \\
    Learning rate & 1e-4 \\
    LR schedule & cosine \\
    LR warmup steps & 10 \\
    LoRA dimension & 8 \\
    Optimizer & Adam \\
    Weight decay & 0.1 \\
    %Prompt loss weight & 0.0 \\
    \bottomrule
    \end{tabular}
    \quad\quad %
    \begin{tabular}[t]{llr}
    \toprule
    \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
    \midrule
    \multirow{5}{*}{Reward model}
    & Epochs & 3 \\
    & Batch size & 128 \\
    & Learning rate & 1e-4 \\
    & LoRA dimension & 8 \\
    & Weight decay & 0.0 \\
    \midrule
    \multirow{8}{*}{Policy model}
    & Epochs & 3 \\
    & Batch size & 32 \\
    & Learning rate & 1e-4 \\
    & LoRA dimension & 8 \\
    & Weight decay & 0.0 \\
    & KL reward coefficient & 0.02 \\
    & PPO clipping parameter & 0.2 \\\
    & Sampling temperature & 1.0 \\
    \bottomrule
    \end{tabular}
\end{table}

==> notes.tex <==
\section{Notes - REMOVE BEFORE SUBMISSION}

\subsection{Data preprocessing implementation details}

\BENJAMIN{
Data preprocessing:
\begin{itemize}
    \item Supervised fine-tuning
    \begin{itemize}
        \item Generate tests
        \item Filter to a ``gold'' set of tests
        \begin{itemize}
            \item Correct syntax
            \item Not empty
            \item Has assertion
            \item Has focal method call
            % \item Has comment?
            % \item Has descriptive signature?
            \item No duplicate assertions
            \item No conditionals or try/catch
        \end{itemize}
        \item Deduplicate on prompt, completion
        \item Filter out prompts and completions which don't fit into the context length
        \item Final number of prompt/completion pairs: {\xxx}
    \end{itemize}
    \item Reward model (RM) fine-tuning
        \item Because babel requires the reward model to be implemented as an LLM, we annotated the prompts and completions with reward scores, then fine-tuned the reward model.
        \item Generate tests
        \item Assign rewards
        \begin{itemize}
            \item Incorrect syntax: -1
            \item Correct syntax:
            \begin{itemize}
                \item Non-preferred: 0
                \item Preferred: 1
            \end{itemize}
        \end{itemize}
        \item Resample to balance classes:
        \begin{itemize}
            \item There are three classes of reward: -1, 0, 1.
            \item Balance the classes between 0 and 1 reward by undersampling the majority class. Dataset $D_{correct} = sample(D_0, d) \cup sample(D_1, d)$ where $d = min(|D_0|, |D_1|)$
            \item For -1 reward, take $D_{incorrect} = \min(|D_{correct}|, D_{-1})$
            \item The final dataset is $D = D_{correct} \cup D_{incorrect}$
        \end{itemize}
        \item Deduplicate on prompt, completion
        \item Filter out prompts and completions which don't fit into the context length
        \item Sample 10,000 prompt/completion pairs
        \item Final number of prompt/completion/reward triples: {\xxx}
    \item Policy model (PM) fine-tuning
    \begin{itemize}
        \item No need to generate tests
        \item Deduplicate on prompt
        \item Sample 1,000 prompts
        \item Final number of prompts: {\xxx}
    \end{itemize}
    \item We initialized RM and PM weights from the SFT weights.
    \begin{itemize}
        \item We found that in practice, fine-tuning the RL model directly resulted in a model which almost invariably predicted.
        \item This is likely because the model was not yet fine-tuned to produce valid tests in response to the prompt. Because the policy model was too unconstrained, it could produce completions which ``hacked'' the reward model, producing high reward while not meeting the static quality metric.
    \end{itemize}
\end{itemize}
}

\subsection{Overall SFT and RL pipeline}
\BENJAMIN{
\begin{itemize}
    \item Generate tests with the Base model
    \begin{itemize}
        \item Use the best inference options and prompting scheme
    \end{itemize}
    \item Split into train/test set on repository
    \item Fine-tune the base model with RL
    \begin{itemize}
        \item Analyze generated tests to count the quality properties.
        \item Assign reward based on the properties. 1 if property is contained, 0 otherwise.
        \item Undersample from the majority class so that the label distribution is balanced.
    \end{itemize}
    \item Evaluate policy model on the test set.
    \begin{itemize}
        \item Mean reward.
        \item Modeled reward.
        \item Proportion of tests with correct syntax.
        \item Proportion of tests containing property.
    \end{itemize}
    \item Evaluate reward model on the test set.
    \begin{itemize}
        \item Mean MSE loss.
    \end{itemize}
\end{itemize}
}

\subsection{Design decisions}
\BENJAMIN{
\begin{itemize}
    \item Penalize incorrect syntax? Yes, though needs to be validated on SFT-first.
    \item Separate data between PPO and RM? Yes, performs better and data are plenty. Needs to be validated on SFT-first.
    \item Subsample/balance label distribution for RM? Not tested.
\end{itemize}
}


==> sections/_02-approach-old.tex <==
\section{Approach}

\subsection{Data collection}

\begin{table}[t]
    \centering
    \caption{Statistics of the dataset of focal methods.}
    \label{tab:dataset-statistics}
    \begin{tabular}{lr}
    \toprule
    \textbf{Statistic} & \textbf{Value} \\
    \midrule
    \# projects                   & 82 \\
    \# focal classes              & 13,567 \\
    \# focal methods              & 62,103 \\
    Mean \# SLOC per focal method       & 6.5 \\
    Mean \# parameters per focal method & 1.6 \\
    \bottomrule
    \end{tabular}
\end{table}

% \BENJAMIN{Paragraph: Dataset}
We constructed our dataset by curating focal methods from open-source C\# projects on GitHub. Initially, we identified 100 non-fork projects predominantly written in C\# with a minimum of 5 stars. Among these, we exclusively considered projects featuring TestMethods written in the MSTest framework, ultimately selecting 82 repositories. From these repositories, we extracted all eligible public methods for test case generation. Our dataset consists of 62k focal methods sourced from these 82 projects, averaging around 757 focal methods per project.


% We collected a dataset of focal methods from open-source C\# projects on GitHub. We selected 100 non-fork projects whose main source code language is  C\# with at least 5 stars. From these, we select only the projects that contain a TestMethod written in MSTest framework, remaining with 82 repositories. From these we extract all the public methods for which we intend to generate a test case. 
% \BENJAMIN{How were projects and focal methods selected?}
% Our dataset contains 62k focal methods, sourced from 82 projects, with an average of 757 focal methods per project.

\subsection{Generating Unit Tests with Language Models}
% \subsection{Test generation}
\label{sec:prompting}

% \BENJAMIN{Paragraph: the setting is to generate one MSTest method.}
We conceptualize the task of unit test generation as completing a test case based on a focal method and its context -- focal class source code and relevant file-level context.
%, namely the other comments, fields, and methods of the class containing the focal method and the surrounding code in the same file.
% \ALEXEY{briefly, what context is that}
To maintain simplicity, we direct the model to generate a single method sequentially using the MSTest format~\cite{MSTest2023}.

% We judged the quality of the test cases along three axes: \textbf{basic properties}, \textbf{best practices}, and \textbf{test smells}.

We generate tests using the OpenAI Codex Cushman model, version \texttt{code-cushman-001}. This version of Codex is a GPT-style model, pretrained on 54 million public repositories using the causal language modeling objective, and has a maximum context length of 2,048 tokens~\cite{chen2021evaluating}.

% \BENJAMIN{Paragraph: Simulated prompt design}
We focused on a specific prompt design, the \textit{``simulated'' prompt}, to harness optimal test generation capabilities from the base Codex model. This prompt design is optimized for code completion, and was chosen because it consistently yielded syntactically correct tests in our desired format (a single MSTest method).
% while circumventing the model's inclination to produce natural language explanations.

% \begin{listing}
%     \begin{minted}{Python}
%         def hello_world():
%             print("Hello floating world!")
%     \end{minted}
%     \caption{Floating listing.}
%     \label{lst:hello}
% \end{listing}

% \begin{listing}
%     \begin{minted}[linenos=true,breaklines,highlightlines={33-37},highlightcolor=green,escapeinside=||]{csharp}
% src/Memstate.Runner/Commands/BenchmarkCommand.cs:
% using System;
% using System.Linq;
% using System.Threading.Tasks;

% namespace Memstate.Runner.Commands
% {
%     public class BenchmarkCommand : ICommand
%     {
%         |\tikzmark{ctxbegin}|private readonly WriteBenchmarkCommand _writeBenchmark = new WriteBenchmarkCommand();

%         private readonly ReadBenchmarkCommand _readBenchmark = new ReadBenchmarkCommand();

%         public event EventHandler Done = (sender, args) => { };

%         public async Task Start(string[] arguments)
%         {
%             await _writeBenchmark.Start(arguments.ToArray());
%             await _readBenchmark.Start(arguments.ToArray());
%         |\tikzmark{ctxend}|}

%         public async Task Stop()
%         {
%             await _writeBenchmark.Stop();
%             await _readBenchmark.Stop();
%         }
%     }
% }

% src/Memstate.Runner/CommandsTestBenchmarkCommand.cs:
% [TestMethod]
% public void TestStop|\colorbox{green}{()}|
% {
%     var command = new BenchmarkCommand();
%     command.Stop().Wait();
%     Assert.IsTrue(command.IsStopped());
% }
% \end{minted}
% \begin{tikzpicture}[overlay, remember picture]
% \node[anchor=base] (a) at (pic cs:ctxbegin) {\vphantom{h}}; % push the mark to the top of the line (ie including ascenders)
% \node[anchor=base] (b) at (pic cs:ctxend) {\vphantom{g}}; % push the mark to the bottom of the line (ie including descenders)
% \draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,gray]
%  (a.north -| {pic cs:right}) -- (b.south -| {pic cs:right});
% \end{tikzpicture}
% % \begin{tikzpicture}[overlay, remember picture]
% % \draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,gray]
% %  ($(right)!(2nd.north)!($(right)-(0,1)$)$) --  ($(right)!(4th.south)!($(right)-(0,1)$)$);
% % \end{tikzpicture}
% \end{listing}

\begin{figure}[t]
    \centering
    % \includegraphics[height=1.5in,page=55]{example-image-duck}
    \includegraphics[height=5in]{figures/Code Example.drawio.pdf}
    
    % \BENJAMIN{This is a mock-up figure showing the prompt with different levels of context labeled, prompt hint with beginning of test method signature highlighted, model completion highlighted with separate background color, and code extraction from model completions.}
    \caption{Our ``simulated'' prompt design for test generation. The context is truncated to fit within the model's context length. The model is tasked with completing a single test method starting with the prompt hint.}
    \label{fig:test-generation-example}
\end{figure}

Figure \ref{fig:test-generation-example} details the simulated prompt design. Our approach emulates the code completion task, which is the closest to the causal language modeling pretraining objective. It's worth noting that code completion models like Codex can struggle with natural-language directions unless specifically fine-tuned to follow such instructions~\citeme{instructgpt}. We emphasize that our findings regarding the effectiveness of RLSQM are orthogonal to prompt design, and can be integrated with a diverse set of prompts. 
As shown in Figure~\ref{fig:test-generation-example}, we construct the prompt as follows (top to bottom):

% \BENJAMIN{Currently, I am double-checking which of these prompts performs the best. We will use instruct-style if it gives similar or better performance compared to the more complex/risky simulate-style.}

% \noindent{\textbf{Instruct-style prompt}}
% \begin{center}
% \begin{tabular}{l}
% \texttt{Given this code:}\\
% \texttt{\textasciigrave{}\textasciigrave{}\textasciigrave{}}\\
% \texttt{\textlangle{}FocalCode\textrangle{}}\\
% \texttt{\textasciigrave{}\textasciigrave{}\textasciigrave{}}\\
% \texttt{Write a C\# unit test using MSTest for the method \textlangle{}FocalMethod\textrangle{}.}\\
% \texttt{Output executable code only.}\\
% \texttt{\textasciigrave{}\textasciigrave{}\textasciigrave{}}\\
% \texttt{public void Test\textlangle{}FocalMethod\textrangle{}}\ldots
% \end{tabular}
% \end{center}

% \begin{enumerate}
%     \item \texttt{\textlangle{}FocalCode\textrangle{}}: The source code of the class containing the focal method.
%     \item \texttt{public void Test\textlangle{}FocalMethod\textrangle{}}: A prompt hint which specifies the beginning of the test method.
%     \item \ldots: The end of the prompt where the model's generation starts.
% \end{enumerate}

% \noindent{\textbf{Simulate-style prompt}}
\iffalse
\begin{center}
\begin{tabular}{l}
\texttt{path/to/FocalClass.cs}\\
\texttt{\textlangle{}FocalCode\textrangle{}}\\
\texttt{path/to/TestFocalClass.cs}\\
\texttt{public void Test\textlangle{}FocalMethod\textrangle{}}
\end{tabular}
\end{center}
\fi

\begin{itemize}
    \item \texttt{path/to/FocalClass.cs}: The path to the file containing the focal method in the actual project structure.
    % \item \texttt{\textlangle{}FocalCode\textrangle{}}: The source code of the class containing the focal method.
    \item \texttt{\textlangle{}ContextAndFocalMethod\textrangle{}}: The source code of the focal method and its context.
    % \item \texttt{path/to/TestFocalClass.cs}: The path to a hypothetical test class for the focal class, adhering to standard project structures.
    % https://stackoverflow.com/a/6295698
    \item \texttt{path/to/TestFocalClass.cs:}$\rhookswarrow$\texttt{\\public void Test\textlangle{}FocalMethod\textrangle{}}: A prompt hint which specifies a hypothetical filepath for the test class and the beginning of the test method signature.
\end{itemize}

% \BENJAMIN{Paragraph: Adaptive context and subsequent filtering of too-long prompts.}
We employ \textit{adaptive focal context} truncation to ensure the inputs fit within the model's context length, similar to the representation introduced in \cite{tufano2021unit}. In detail, we adopt a sequential approach to extract focal contexts, where each next option is a more concise representation than its predecessor:
\begin{enumerate}
\item Entire text of the focal file, which can include imports, namespaces, and other classes.
\item Focal class code, converting methods other than the focal method into their respective signatures.
\item Focal class code, converting non-focal methods to signatures and eliminating fields/comments.
\item A stripped-down version comprising only the focal class definition and focal method, while discarding all supplementary code.
\item Prompts persistently exceeding the permitted length were removed.
\end{enumerate}
We try these focal context alternatives until the resulting prompt fits the context window of the LLM.

% \BENJAMIN{Code extraction - extract first method and do simple cutting on closing brace and [TestMethod] annotation.}
The LLM-generated completions might contain multiple test methods. To isolate a single test method from the model's output, we truncate any tokens generated by the model following the second occurrence of the \texttt{[TestMethod]} – an annotation signifying the beginning of a new test method -- or the closing brace \texttt{\}}, occurring on a new line without indentation, marking the end of the test method. 

\begin{table}[htbp]
    \centering
    \caption{Nucleus sampling parameters for test generation}
    \label{tab:test_generation_parameters}

    \begin{tabular}{lr}
    \toprule
        \textbf{Parameter} & \textbf{Value} \\
    \midrule
        Temperature & 0.7 \\
        top\_p & 1.0 \\
        Frequency penalty & 0.5 \\
        Prompt length & 1,536 \\
        Completion length & 512 \\
    \bottomrule
    \end{tabular}
\end{table}

% \BENJAMIN{Paragraph: Motivation of hyperparameters}
We generated tests using nucleus sampling~\cite{Holtzman2020The} with parameters listed in Table \ref{tab:test_generation_parameters}.
We used a temperature setting of 0.7 and generated multiple completions for each prompt in order to generate diverse test code.
We noted that Codex tended to generate repeated assertions or comments and therefore overrun the maximum context length, resulting in an incomplete and syntactically incorrect method. To alleviate this problem, we set the frequency penalty to 0.5 to discourage the model from generating tokens which have already been sampled~\footnote{For details, see \url{https://platform.openai.com/docs/api-reference/chat/create\#frequency_penalty}.}.
In order to give the maximum context while allowing the model to generate complete tests which are long enough to be useful, we limited completions to 512 tokens and allowed the context to fill the remaining 1,536 tokens -- this equates to roughly 6,144 characters of context~\footnote{\url{https://platform.openai.com/tokenizer}}. In our dataset, we measured about 45 source lines of code (SLOC) in each prompt on average~\footnote{using \url{https://github.com/XAMPPRocky/tokei}}.
We removed less than 0.1\% focal methods in our dataset as too long.
% \BENJAMIN{Consider deferring the specific number of tests generated because it depends on later implementation details which differ between RQ1 and RQ2.}
% Our dataset contains 62k focal methods, which we filtered to \xxx{} focal methods which fit inside the context length.
% We generated 100 tests for each focal method, resulting in a dataset of \xxx{} generated tests.

\subsection{Evaluating Test Case quality}
Given the dataset of prompts (focal code with annotations, and the beginning of the test method signature) and their respective unit tests obtained in Section~\ref{sec:prompting}, we assess the properties of the generated unit tests with respect to the coding best practices (e.g. syntax correctness) and evaluate for presence of test-smells. Namely, a good quality unit test should have at least one assert statement, an invocation of the focal method, and have a descriptive signature. See Section \ref{sec:rq1} for details on assessing the test case static quality metrics.
To detect these quality metrics, we implement a tool which we call ``Quality Analyzer'' using the tree-sitter parser~\cite{treesitter} to analyze the unit test properties. The results of the analysis provide insights into the quality metrics that needed improvement, ensuring the model can produce high-quality test cases. The Quality Analyzer serves as a foundation for construction of the datasets for supervised fine-tuning and RL training in our RLSQM approach.


%\MICHELE{I would suggest move out some of the content from the RL subsection into their corresponding subsections here. After we generate the tests from tbe baseline codex, we evaluate the test properties. Not sure yet if we want to descibe all of them here or in the RQ1, but we have a clear step. We may just want to say that at this level we implemented a tool that anlyzes the qualities and properties of test cases}


\subsection{Supervised Fine-tuning}
Building on the output of the prior step -- a collection of generated tests with static quality metrics -- we initiate the creation of the \textit{golden dataset} for supervised finetuning. Within this dataset, every unit test must exhibit syntactic correctness, contain at least one assertion, and invoke the focal method, while avoiding duplicate assertions and conditionals. We curate this dataset, isolating the gold standard of test cases that embody optimal qualities, adhere to best practices, and avoid test smells. Section~\ref{sec:rq2} provides more details on the unit test static quality metrics.

The language model is then fine-tuned to maximize these optimal qualities by minimizing the cross-entropy loss, expressed as follows:
\begin{equation}
    L_{CE} = -\sum_i^n \log{P(w_i | w_1, \ldots, w_{i-1})}
\end{equation}
Here, $w_1, \ldots, w_{m}$ are the prompt tokens, and $w_{m+1}, \ldots, w_{m+n}$ are the tokens of the completion. Figure \ref{fig:sft} illustrates the supervised finetuning process. It is important to emphasize that the curation of the golden dataset for SFT is automatic, without any manual labeling or intervention by human experts. 

By filtering the dataset to only include test cases with desirable qualities, we are effectively \textit{refining} the model to generate higher-quality test cases. Although SFT on the golden dataset of unit tests produces higher quality test cases, our experimental results (discussed in Section \ref{sec:rq2}) highlight the limitations of this approach. In contrast to SFT, reinforcement learning allows the model to learn from unfavorable examples and actively penalize undesirable behaviors and test smells, offering a more robust training process.


\begin{figure}
    \centering
    % \includegraphics[height=1.5in,page=10]{example-image-duck}
    \includegraphics[width=1.0\textwidth]{figures/sft_rm_ppo.pdf}

    \caption{Overview of supervised fine-tuning. \MICHELE{Just temporary. Should we place a single figure with all the stages, or smaller figures for each stage?}}
    \label{fig:sft}
\end{figure}



\begin{figure}
    \centering
    % \includegraphics[height=1.5in,page=10]{example-image-duck}
    \includegraphics[width=1.0\textwidth]{figures/sft.pdf}

    \caption{Overview of supervised fine-tuning. Starting with a foundational Codex LLM and a golden set of input prompts and high-quality unit tests, we update the model weights, through the standard stochastic gradient descent optimization procedure. Hyperparameters used during SFT training are listed in Table~\ref{tab:training-parameters} (left).}
    \label{fig:sft}
\end{figure}


\subsection{Reinforcement Learning from Static Quality Metrics}
% \MICHELE{Finally, we perform RL part}

\input{figures/sft-rl-parameters}

Reinforcement learning has been successfully applied to natural language and code generation tasks to avoid the exposure bias induced by teacher forcing~\citeme{}. RL can directly optimize models for metrics evaluated during inference and can leverage nuanced human feedback. In the Reinforcement Learning from Static Quality Metrics (RLSQM) framework, we apply RL to the task of unit test case generation. In this application, the learning process is a variant of an episodic RL scenario~\citeme{}. In our scenario, the agent, operating within an environment tailored to code generation, aims to produce unit test cases by sequencing tokens from an action space, which is the vocabulary of tokens $\mathcal{V}$. The observation space in this context refers to all possible prompts, from which a unit test case needs to be completed. As the agent navigates this space, it relies on a policy $\pi$, instantiated by a pretrained language model, to decide its next action. This policy provides a distribution over tokens, which seeks to guide the agent in making decisions that maximize the episodic reward. 
In this scenario, the agent receives a reward $\mathcal{R}$ at the end of the episode, which corresponds to the successful completion of a unit test case. 

\subsubsection{PPO Fine-tuning}
RLSQM utilizes the Proximal Policy Optimization (PPO)~\cite{ppo} algorithm, to refine the agent's actions. We use a variant of PPO which integrates both the clipped objective and the Kullback-Leibler (KL) penalty modulated by the KL reward coefficient $\kappa_{\text{KL}}$. PPO operates as an actor-critic algorithm, combining two instrumental parts: the actor, determining the policy $\pi$, and the critic, valuing a given state-action pair to better the actor's choices. This dual-network method guarantees that policy updates are restrained, averting excessively bold policy changes which might disrupt training. The PPO's objective utilized in RLSQM is represented as:
\begin{equation}
L(\theta) = L^{\text{CLIP}}(\theta) + \lambda \times L^{\text{KL}}(\theta)
\end{equation}

Where \( L^{\text{CLIP}}(\theta) \) embodies the clipped objective:
\begin{equation}
L^{\text{CLIP}}(\theta) = \mathbb{E}\left[ \min \left( r_t(\theta) A^{\text{old}}(s_t, a_t), \text{clip}\left(r_t(\theta), 1-\epsilon, 1+\epsilon\right) A^{\text{old}}(s_t, a_t) \right) \right]
\end{equation}

Simultaneously, \( L^{\text{KL}}(\theta) \) represents the KL divergence penalty:
\begin{equation}
L^{\text{KL}}(\theta) = \mathbb{E}_{t}\left[ D_{\text{KL}}(\pi_{\theta_{\text{old}}}, \pi_{\theta}) - \kappa_{\text{KL}}
 \times \hat{R}_t \right]
\end{equation}

Where the ratio \( r_t(\theta) = \frac{\pi_\theta(a_t|s_t)}{\pi_{\theta_{\text{old}}}(a_t|s_t)} \) contrasts the new policy's probability to the old's for action \(a_t\) in state \(s_t\), \( A^{\text{old}}(s_t, a_t) \) is the advantage estimate from the old policy, and $\epsilon$ is a PPO clipping parameter that confines the policy's update magnitude. The term $D_{\text{KL}}$ denotes the KL divergence. Figure~\ref{fig:ppo} provides the details on the RLSQM's PPO finetuning stage. \ALEXEY{changed to kl\_rew\_coef version of PPO, need to double check the formulas}

It is worth noting that our approach is not tied to the PPO algorithm and implementations may employ a variety of other reinforcement learning algorithms, such as A2C~\citeme{} or NLPO~\citeme{}.

\subsubsection{Reward Model Training}
As in the RLHF, the reward model (RM) is pivotal to our approach. However, rather than relying on human feedback, we employ a static Quality Analyzer to determine rewards. These derived rewards are then harnessed to train a model to estimate expected rewards from the agent's decisions. This RM training process optimizes the Mean Squared Error (MSE) loss, expressed as:
\begin{equation}
\text{MSE} = \frac{1}{n} \sum_{i=1}^{n} (y_i - \hat{y}_i)^2
\end{equation}

In this equation, \(y_i\) is the reward as per the Quality Analyzer, and \(\hat{y}_i\) is its predicted counterpart.
% Through this mechanism, the RM incessantly sharpens its predictions, granting the agent a precise read on feedback and enhancing policy optimization.
By minimizing the MSE, the RM learns to predict a score that closely matches the Quality Analyzer, even when evaluating unseen tests.
Figure~\ref{fig:reward_model} zooms in at the RLSQM reward model finetuning stage.

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/rm.pdf}

    \caption{Overview of Reward Model training. We generate completions using the supervised fine-tuned model, then train the reward model to predict quality scores output by our Quality Analyzer. Hyperparameters used during RM training are listed in Table~\ref{tab:training-parameters} (top right).}
    \label{fig:reward_model}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/ppo.pdf}

    \caption{Overview of Policy Model training. We initialize the policy model with th supervised fine-tuned weights, then further train it to maximize rewards predicted by the Reward Model. Hyperparameters used during the PPO finetuning training are listed in Table~\ref{tab:training-parameters} (bottom right).}
    \label{fig:ppo}
\end{figure}

% \BENJAMIN{Fill in the rest of the approach. Should we introduce individual, then multi-rewards? How best to do this?}




==> sections/ablations.tex <==
% \section{RQ$_3$: Effects of Individual and Multiple Reward Training}
\section{Effects of Individual and Multiple Reward Training}
\label{sec:rq3-results}

To study the effects of training with single rewards versus multiple rewards, we trained RLSQM in an array of configurations using Individual, Sequential, and Combined Rewards and evaluated each configuration on syntactic correctness and overall test quality.
For Individual Rewards, we trained a model for each quality property. The results show that RLSQM was most effective for Best Practices and Test Smells, so we focused on these properties when training multiple rewards.
For Sequential Rewards, we trained a new quality property in the \nth{2} stage.
For Combined Rewards, we evaluated all combinations of 2, 3, or 4 properties.

% \ben{Move to appendix, summarize ablation in text}

% \begin{table}[t]
%     \centering
%     \caption{Quality metrics on the test set after RL fine-tuning with Individual Rewards.
%     \goodmark{} denotes positive features which should be encouraged; \badmark{} denotes negative features which should be discouraged.
%     Improvement/regression on each property is compared to the SFT model. \colorbox{yellow!50}{Highlighted cells} denote the properties under optimization. RL models are compared to the SFT baseline\textsuperscript{\ref{footnote:dataset-difference}}.
%     % \BENJAMIN{Add a column for the test cases' compile/pass rate.}
%     % \BENJAMIN{This result includes manually selected checkpoints for Comments and Try/Cond, which were picked to be the latest checkpoints before large variance of KL/pertok. This rule must be formalized and explained in the final draft.}
%     % \BENJAMIN{This result includes checkpoints selected by validation performance, Overall.} \MICHELE{I know I suggested this graphic, but do you think it may be unnecessary? Should we just report the percentages?}
%     }
%     \label{tab:individual-rewards}
%     % \input{figures/individual-rewards}
%     \vspace{-1em}
% \end{table}
\begin{figure}[h]
    \centering
    \begin{tabular}{cc}
        \multicolumn{2}{c}{Improvement} \\
        \colorsquare{SFT_Doc} Yes & \colorsquare{GPT4} No \\
    \end{tabular}
    \includegraphics[width=\linewidth]{figures/individual.png}
    \begin{tabular}{@{\hskip 0.5in}c@{\hskip 0.25in}c@{\hskip 0.15in}c}
    \goodmark{} Best Practices &
    \badmark{} Test Smells &
    \goodmark{} Documentation
    \end{tabular}
    \caption{Effects of RLSQM fine-tuning with Individual Rewards. We report change relative to Base Codex.
    The intended outcome is to reduce negative \badmark{} Test Smells and increase positive properties like \goodmark{} Best Practices. 
    % \goodmark{} denotes positive features which should be encouraged; \badmark{} denotes negative features which should be discouraged.
    % Improvement/regression on each property is compared to the SFT model. \colorbox{yellow!50}{Highlighted cells} denote the properties under optimization. RL models are compared to the SFT baseline\textsuperscript{\ref{footnote:dataset-difference}}.
    }
    \label{tab:individual-rewards}
    \vspace{-1em}
\end{figure}

% \BENJAMIN{Concise, update after removing table}
Figure \ref{tab:individual-rewards} shows the change in the frequency of each quality property after Individual Reward training, compared with the Base model.
RLSQM improved the four Best Practices and Test Smells, notably increasing the frequency of Assertions up to 92.8\% and nearly eradicating Conditional/Exception tests (down to 0.16\% frequency).
% 
% Some interesting findings
By learning from negative examples with incorrect syntax, RL fine-tuning substantially increased the syntactic correctness of their generations, with all RLSQM models achieving 97-99.5\% syntactic correctness. Qualitatively, RL models avoided failure modes such as repeated assertions and comments, which frequently caused the Base and SFT models to generate incomplete tests.

Interestingly, for some properties, the model which optimized one property did not perform as well on that property as a model which optimized another property.
For example, the \ppomodel{\goodmark{} Focal Call} model produced more tests with Assertions than the \ppomodel{\goodmark{} Assertion} model. This may be due to correlation of these properties in the reward model training data, resulting in a RM which learns to reward both properties in a secondary nature.
In our dataset, 34\% of Focal calls occur as arguments to Assertions; therefore, a model that rewards Focal calls may also learn to include the Assertions which commonly wrap them.
Although joint optimization is beneficial in this case and many others, future work can attempt to optimize these properties precisely, without the effect of such correlations.


RLSQM produced fewer Documentation properties than the Base model, which may be due to initialization with SFT weights. We leave addressing this limitation to future work and focus subsequent experiments on optimizing Best Practices and Test Smells.

% The rows corresponding to the RL models also show the improvement/regression compared to the SFT model, from which the RL optimization was performed.
% \BENJAMIN{TODO: Note differences from Table \ref{tab:test_properties}.
% RQ1 evaluates models on the entire dataset while RQ2-3 holds out data for training and evaluates all models on a test dataset made of projects which are separate from the training dataset; the observed variability is expected on a subset of the data.}

% \renewcommand*{\thefootnote}{\arabic{footnote}}
% GPT-4 was selected as our strongest LLM baseline, generating high-quality tests across all dimensions and properties investigated. GPT-4 produced tests with more Descriptive Names (23\%), more Comments (78\%), and fewer Duplicate Assertions (0.55\%) than the Codex-based models (Base). Since GPT-4 is trained to understand and generate human-like code~\cite{gpt4}, it's not surprising that it produced documentation and avoid consecutive duplicated assertions.
% We estimate that fine-tuned Codex is several orders of magnitude smaller and costs less than half as much as GPT-4\footnote{Up-to-date pricing information is no longer available for code-cushman-001 (12B parameters); however, at less than one-tenth the size, we conservatively estimate that RLSQM will cost much less than fine-tuned davinci-002 (175B) at \$0.012/KT (thousand-tokens), which costs less than half of GPT-4 at \$0.03/KT (\url{https://openai.com/pricing}).}, and thus can be deployed to generate less-smelly tests at lower cost.
% \renewcommand*{\thefootnote}{\fnsymbol{footnote}}

% The SFT model improved upon the Base model in all properties except Descriptive Names and Comments, but it could not be optimized beyond a certain point. The model likely regressed on Descriptive Names and Comments because these properties were not selected in the golden training set due to regression on the other properties.
% The Base model generated these properties relatively infrequently, so when we used them to filter the SFT training set, the dataset was much smaller. The resulting model improved on these two properties but performed worse than the Base model on the \new{Syntax, Best Practices, and Test Smell properties; we discuss its performance alongside Table \ref{fig:performance-summary}}.
% % \BENJAMIN{Refer to new table showing these results.}.
% Therefore, we chose to initialize the RL models from the SFT model which ignored Documentation properties.
% This highlights a limitation of the SFT training regime -- the approach performed sub-optimally when the desired properties restricted the golden training dataset.

% Moved to Setup.
% % \new{The Base model generated Documentation properties (Descriptive Names and Comments) relatively infrequently (\S~\ref{sec:rq1}), so when we used them to filter the SFT training set, the dataset was over 50x smaller.
% The Base model generated Documentation properties relatively infrequently (\S~\ref{sec:rq1}), which made the SFT training set 50x smaller.
% The resulting model, which we call SFT$_{\text{Doc}}$, improved on the two Documentation properties but performed worse than the Base model on the other five properties; we discuss its performance in Table \ref{fig:performance-summary}.
% We continue with the SFT model filtered only on Necessary/Best Practices and Test Smells, which regressed on Documentation properties but improved all the others compared to the Base model.
% This highlights a limitation of the SFT training regime -- the approach performed sub-optimally when the desired properties restricted the golden training dataset.

% RLSQM improved most properties under optimization, yielding models that consistently outperformed Base, SFT, and GPT-4 across the quality metrics we examined.

% The only exception pertains to Descriptive Names and Comments, with both properties decreasing by 1.6\% and 10.1\% compared to SFT, respectively. We hypothesize that the initial weights provided by the SFT model, which tended to reduce Documentation properties (note Documentation properties decreasing from Base to SFT in Table \ref{tab:individual-rewards}), constrained the policy model's ability to enhance these specific properties. Incorporating these properties necessitates the model's transition from code to natural language at precise locations, a behavior that may pose challenges for the policy model to explore effectively. This is also supported by the fact that, without validation and proper setting of the KL reward coefficient, the policy model tended to generate long, un-terminated comments which overran the context length, resulting in a syntactically incorrect, incomplete test. We leave exploration of these properties to future work and focus our analysis in the following section on the Best Practices and Test Smells, which showed promising improvement from RL fine-tuning.

% \BENJAMIN{Summarize in one sentence.}
% Reinforcement-learning models were able to increase all quality metrics above those of the SFT model and often outperformed GPT-4, indicating that RLSQM fine-tuning was capable of enhancing individual quality metrics. Specifically, RLSQM increased by +7.9\% the presence of asserts, +10.9\% the invocation of the correct focal method, and contributed to the reduction of test smells by decreasing duplicate asserts by -0.14\% and diminishing the presence of conditional logic in test cases by -0.07\%.
% Additionally, by learning from the examples with incorrect syntax, RL models were able to substantially increase the syntactic correctness of their generations, close to 100\%. By our observations, the RL models avoided failure modes such as repeated assertions and comments, which frequently caused the Base and SFT models to generate incomplete tests.

% \BENJAMIN{Summarize in two sentences, merge with discussion of doc properties as "discussion".}
% For some properties, the model which optimized one property did not perform as well on that property as a model which optimized another property. For example, the Assertion property was outperformed by the model optimizing \ppomodel{\goodmark{} Focal Calls} than the model optimizing \ppomodel{\goodmark{} Assertions}. This may be due to the reward model optimizing these properties in a secondary nature, and may be due to correlation of the properties in the reward model training data.
% \BENJAMIN{More digging necessary here. Also consider that the properties themselves may be correlated, such as focal method calls inside assertion statements.}
% In this instance, 34\% of Focal calls occur as arguments to Assertions; therefore, a model that learns to reward Focal calls may also learn to include the Assertions which commonly wrap them.
% Future work can attempt to optimize these properties precisely, without the effect of such correlations.

% Overall, RL from Individual Rewards (optimizing \ppomodel{\badmark{Duplicate Assertions}}) improved upon the Base model by increasing best practices: up to $\uparrow$ 21.4\% Assertions and $\uparrow$ 18.9\% Focal calls, and reducing test smells: up to $\downarrow$ 1.4\% Duplicate Assertions and $\downarrow$ 2.4\% Conditionals/Exceptions.

% \setlength\fboxsep{2pt}
% \vspace{-0.05cm}
% \begin{center}
% \colorbox{gray!20}{
% \begin{minipage}[t]{0.97\linewidth}
% {\bf Summary for RQ$_2$.}
% Overall, RL from Individual Rewards (optimizing \ppomodel{\badmark{Duplicate Assertions}}) improved upon the Base model by increasing best practices: up to $\uparrow$ 21.4\% Assertions and $\uparrow$ 18.9\% Focal calls, and reducing test smells: up to $\downarrow$ 1.4\% Duplicate Assertions and $\downarrow$ 2.4\% Conditionals/Exceptions.
% \end{minipage}
% }
% \end{center}
% \setlength\fboxsep{0pt}




% RLSQM improved all properties under optimization, except for Descriptive Names and Comments -- these properties were substantially reduced compared to SFT, decreasing by 1.6\% and 10.1\% respectively.



% However, all of the RL-trained models were able to perform better on Assertions Focal Calls, and Conditional/Exceptions, including up to 8.5{}\% improvement on Syntax and 15.4\% improvement on Asserts.

% RL improved all properties under optimization, except for Descriptive Names and Comments -- these properties were substantially reduced compared to SFT, decreasing by 1.6\% and 10.1\% respectively.


% Table \ref{tab:individual-rewards} shows the frequency of each quality metric, as well as the improvement/regression compared to the SFT model.
% RL improved all properties under optimization, except for Descriptive Names and Comments -- these properties were substantially reduced compared to SFT, decreasing by 1.6\% and 10.1\% respectively.
% Although the reward model was able to predict the scalar reward nearly perfectly, the policy model did not generate more tests containing comments.
% \BENJAMIN{May need review - also consider failure mode where the model generates too-long comments.}
% We hypothesize that since the SFT model already tended to decrease the amount of Documentation properties (discussed below), the policy model was not able to explore enough to increase these properties. These properties require the model to switch from code to natural language at specific locations, a behavior which could be difficult for the policy model to explore.
%: immediately after the prompt hint (for Descriptive Names) or inside comment markers \texttt{//} or \texttt{/* */} (for Comments).
% This is also supported by the fact that, without validation and proper setting of the KL reward coefficient, the policy model tended to generate long, un-terminated comments which overran the context length, resulting in a syntactically incorrect, incomplete test.
% We leave exploration of these properties to future work and focus our analysis in the following section on the other properties which showed promising improvement from RL fine-tuning.

% The SFT model improved upon the Base model in all properties except Descriptive Names and Comments, but it could not be optimized beyond a certain point. The model likely regressed on Descriptive Names and Comments because these properties were not selected in the golden training set due to regression on the other properties.
% The Base model generated these properties far less frequently, so when the SFT training set was much smaller and the resulting model tended to improve on these two properties but performed worse than the Base model on the Syntax, Assertion, and Focal call properties. Therefore, we chose to initialize the RL models from the SFT model which ignored Documentation properties.
% This highlights a limitation of the SFT training regime -- the approach performed sub-optimally when the desired properties restricted the golden training dataset.

% Reinforcement-learning models were able to increase all quality metrics above those of the SFT model, indicating that RL fine-tuning was capable of enhancing individual quality metrics.
% Additionally, by learning from the examples with incorrect syntax, RL models were able to substantially increase the syntactic correctness of their generations, nearly to 100\%. By our observations, the RL models avoided failure modes such as repeated assertions and comments, which frequently caused the Base and SFT models to generate incomplete tests.
% \BENJAMIN{Highlight the fact that the SFT model improved compared to Base, but could not optimize past a certain point.}
% \BENJAMIN{The PPO model also has much more correct syntax... Nearly 100\% of generated tests were syntactically correct.}

% For some properties, the model which optimized the property did not perform as well as a model which optimized another property. For example, the \ppomodel{\goodmark{} Asserts} property was improved more by the model optimizing the \ppomodel{\goodmark{} Focal Calls} than the model optimizing the Assert property. This may be due to the reward model optimizing these properties in a secondary nature, and may be due to correlation of the properties in the reward model training data.
% % \BENJAMIN{More digging necessary here. Also consider that the properties themselves may be correlated, such as focal method calls inside assertion statements.}
% For instance, \BENJAMIN{34\% -- quick query but needs verification} of Focal calls occur as arguments to Assertions; therefore, a model that learns to reward Focal calls may also learn to include the Assertions which commonly wrap them.
% Future work can attempt to optimize these properties precisely, without the effect of such correlations.

% GPT-4 produced more Descriptive Names (23\%), more Comments (78\%), and fewer Duplicate Assertions (0.55\%) than the Codex-based models. Since GPT-4 is trained to understand and generate human-like code~\cite{gpt4}, it's not surprising that it produced documentation and avoid consecutive duplicated assertions. However, all of the RL-trained models were able to perform better on Assertions Focal Calls, and Conditional/Exceptions, including up to 8.5{}\% improvement on Syntax and 15.4\% improvement on Asserts. \BENJAMIN{More discussion available?}

% \BENJAMIN{Discuss GPT-4 results. GPT-4 produced more descriptive names (23\%) and more comments (78\%) than Base and RL models.}

% \BENJAMIN{Don't focus too much on best model since this recommendation does not make sense intuitively. Emphasize that all are improvements over SFT and base.}
% Overall, RL from Individual Rewards (optimizing \ppomodel{\badmark{Duplicate Assertions}}) improved upon the Base model by increasing best practices: up to $\uparrow$ 21.4\% Assertions and $\uparrow$ 18.9\% Focal calls, and reducing test smells: up to $\downarrow$ 1.4\% Duplicate Assertions and $\downarrow$ 2.4\% Conditionals/Exceptions.




% \BENJAMIN{Discuss compile/pass results}

% \subsection{RQ$_3$: Improving Overall Test Generation Quality}
\label{sec:rq3}



\noindent\textbf{Sequential Reward:}
Table \ref{tab:iterative-reward} shows the outcomes of Sequential Reward training.
% This shows that the \nth{2} stage of RL training could not reliably improve secondary quality properties.
% 
The properties Assertion and Duplicate Assertion were the most successful, improving in the \nth{2} stage in 5/6 settings.
For 3/4 properties excluding Duplicate Assertions, the \nth{2} stage of RL fine-tuning mostly retained or improved upon the improvements from the \nth{1} stage.
However, compared to the corresponding Individual Reward settings, 6/12 of quality metrics that were optimized in the \nth{2} stage improved or remained nearly unchanged and 6/12 regressed.
While these results show some initial success, further research could seek to more reliably improve the model with Sequential Reward training.

\setlength\fboxsep{2pt}

\begin{table}[t]
    \centering
    \caption{Effects of RLSQM fine-tuning with multiple rewards.
    % 
    \textcolor{black!30!green}{Green text} indicates improvement while \textcolor{black!20!red}{red text} indicates regression, relative to the corresponding \nth{1}-stage Individual Reward model.
    }
    \begin{subtable}[t]{0.48\textwidth}
    \caption{Effects of Sequential Rewards.
    % Each property is compared to the corresponding first-stage Individual Reward model.
    % The properties optimized in the \nth{1} stage are marked \colorbox{yellow!50}{yellow}; properties optimized in the \nth{2} stage are marked \colorbox{orange!50}{orange}.
    \colorbox{yellow!50}{Yellow cells} mark the properties optimized in the \nth{1} stage; \colorbox{orange!50}{Orange cells} likewise for the \nth{2} stage.
    % \colorbox{yellow!50}{Yellow cells} denote the properties under optimization in the \nth{1} stage; \colorbox{orange!50}{Orange cells} denote the properties under optimization in the \nth{2} stage.
    % \textcolor{black!30!green}{Green text} indicates improvement while \textcolor{black!20!red}{red text} indicates regression, compared to the corresponding first-stage Individual Reward model.
    % \BENJAMIN{Color the absolute percentage and remove deltas.}
    }
    \label{tab:iterative-reward}
    % \resizebox{!}{0.5\textheight}{
    % \scalebox{0.9}{
    \input{figures/iterative-reward}
    % }
    \end{subtable}
    % \hspace{200em}
    
    \begin{subtable}[t]{0.48\textwidth}
    \caption{Effects of Combined Rewards.
    % Each property is compared to the corresponding Individual Reward model.
    \colorbox{yellow!50}{Yellow cells} mark the properties under optimization.
    % Green text indicates improvement while red text indicates regression, compared to the best-performing Individual Reward model.
    % \BENJAMIN{Row ``Individual reward'' will list baseline against which the improvement/regression is measured: either the property under optimization in individual reward training, or the best score from all individual reward training runs (even if the property was not being optimized).}
    }
    \label{tab:additive-reward}
    \input{figures/additive-reward}
    \end{subtable}
    \vspace{-1em}
\end{table}

% \BENJAMIN{Summarize in one sentence. BLUF}
% In 7/12 cases, the property optimized in the \nth{1} stage improved and in 5/12 cases, the property regressed; on the other hand, with the exception of Duplicate asserts which regressed from the 1st stage in all cases, the other 3 properties mostly retained their score in the 1st stage.
% In other words, for three out of the four properties optimized, the second stage of RL fine-tuning retained the improvements from the first stage.
%\BENJAMIN{Can we investigate the Duplicate asserts reward model to see why it failed to produce good models?}

% \BENJAMIN{Inspired by RLAIF... can we measure how the quality metrics change from stage 1 and 2? Does the quality of the dataset improve? Why don't we see improvement across the board? Is there an order to these properties, and would there be a best curriculum?}

% \BENJAMIN{Summarize in one sentence.}
% Sequential Reward was able to monotonically improve the model in the setting \ppomodel{(\goodmark{} Focal $\rightarrow$ \badmark{} Conditional/Exception)}, which improved or retained its performance on all quality metrics compared to Individual Rewards. Further fine-tuning would seek to further improve the model by optimizing different properties in subsequent stages.

% \begin{table}[t]
%     \centering
%     \caption{Effects of RLSQM fine-tuning with Combined Rewards.
%     % Each property is compared to the corresponding Individual Reward model.
%     \colorbox{yellow!50}{Highlighted cells} denote the properties under optimization.
%     % Green text indicates improvement while red text indicates regression, compared to the best-performing Individual Reward model.
%     % \BENJAMIN{Row ``Individual reward'' will list baseline against which the improvement/regression is measured: either the property under optimization in individual reward training, or the best score from all individual reward training runs (even if the property was not being optimized).}
%     }
%     \label{tab:additive-reward}
%     \input{figures/additive-reward}
% \end{table}

%%%%%% New combined reward explanation - focus on
% 1. Improvements and why they improved
% 2. Limitations/regression, why they didn't work, why this is OK and we can still train a good model 
% 3. Which model we chose for best RLSQM

\noindent\textbf{Combined Reward:}
Table \ref{tab:additive-reward} shows the results of Combined Reward training.
% 
Two settings improved on all quality properties: \ppomodel{(\goodmark{} Assert + \badmark{} Conditional/Exception)} and \ppomodel{(\goodmark{} Focal + \badmark{} Duplicate assert + \badmark{} Conditional/Exception)}.
Notably, the properties optimized by these models are not intuitively correlated or dependent on each other (compared to e.g. Asserts and Duplicate Asserts, which are certainly interdependent), which may indicate that the Combined Reward setting works most effectively when there are fewer dependencies or potential conflicts between the optimized properties.
% 

However, Combined Reward yielded mixed improvement compared to Individual Reward fine-tuning.
On 2-property optimization, 6/12 optimized properties improved and 6/12 regressed;
on 3-property optimization, 4/9 optimized properties improved while 5/9 regressed;
finally, optimizing All Properties in one reward model performed worse than some 2- or 3-property settings.
The Assert property improved in almost all cases, while the Focal, Duplicate Assert, and Conditional/Exception properties regressed in more than half of the cases.
Along with potential conflicts between quality properties mentioned previously, we hypothesize that this may be because the space of possible rewards grows as more properties are added, ranging from -1 to 4, and thus the policy model got stuck in a local minimum which earned relatively high reward from the reward model, failing to find a balance between exploration and exploitation.
Future work could leverage \textit{reward shaping}~\cite{sutton2018reinforcement} to address this exploration problem.

\noindent\textbf{Summary of RLSQM Training Strategies:}
Overall, RL-finetuned models consistently improved over the Base Codex. The highest-performing model overall was \ppomodel{(\goodmark{} Focal + \badmark{} Conditional/Exception)}, trained with Combined Reward, which substantially improved on all Basic Properties and Test Smells compared to both Codex and GPT-4 (see Section \ref{sec:rq2-results} for a detailed comparison).

% $\uparrow$ 23.2\% Assertions, $\uparrow$ 17.9\% Focal calls, $\downarrow$ 2.22\% Duplicate Assertions, and $\downarrow$ 2.53\% Conditionals/Exceptions; however, it produced 6.1\% fewer tests with Descriptive names and 11.0\% fewer tests with Comments.
% This model also improved on all Basic Properties and Test Smells compared to the GPT-4 model: $\uparrow$ 15.3\% Assertions, $\uparrow$ 0.3\% Focal calls, $\downarrow$ 0.01\% Duplicate Asserts, and $\downarrow$ 2.48\% Conditionals/Exceptions.

% 
% On 2-property optimization, 6/12 optimized properties improved and 6/12 regressed, compared to the corresponding Individual Reward settings.
% On 3-property optimization, 4/9 optimized properties improved while 5/9 regressed. Some properties regressed substantially, such as the Assert and Focal properties in the \ppomodel{(\goodmark{} Assert + \goodmark{} Focal + \badmark{} Conditional/Exception)} setting; we observed this can occur due to the policy model diverging from the starting weights in order to increase the modeled reward.
% The Assert property improved in almost all cases, while the Focal, Duplicate Assert, and Conditional/Exception properties regressed in more than half of the cases.

% By comparing the results of 3-property configurations with 2-property configurations, we see that adding a third property to the reward model often did not cause the policy model to improve on that property. For example, comparing \ppomodel{(\goodmark{} Assert + \goodmark{} Focal)} with \ppomodel{(\goodmark{} Assert + \goodmark{} Focal + \badmark{} Duplicate assert)}, the latter model generated \textit{more} duplicate assertions than the former. The additional property may make the modeled reward more difficult to optimize, preventing the policy model from discovering an optimal policy.

% Similarly, optimizing All Properties in one reward model performed worse than some 2- or 3-property settings. This may be because the space of possible rewards is larger, ranging from -1 to 4, and thus the policy model was not able to sufficiently optimize its completions but got stuck in a local minimum which earned relatively high reward from the reward model.

% \BENJAMIN{Summarize in one sentence. Merge with the following paragraph but still make the point about synergy.}
% In the Combined Reward setting, two settings improved on all properties: \ppomodel{(\goodmark{} Assert + \badmark{} Conditional/Exception)} and \ppomodel{(\goodmark{} Focal + \badmark{} Duplicate assert + \badmark{} Conditional/Exception)}.
% Notably, the properties optimized by these models are not likely to be correlated or dependent (compared to e.g. Asserts and Duplicate Asserts, which are certainly interdependent), which may indicate that the Combined Reward setting works most effectively when there are fewer dependencies between properties.

% \BENJAMIN{Summarize in one sentence. Remove redundancy from RQ2.}
% Observing the best models trained with the Combined and Sequential Reward strategies, we see that RL-finetuned models consistently improved over the Base Codex. The highest-performing model overall was \ppomodel{(\goodmark{} Focal + \badmark{} Conditional/Exception)}, trained with Combined Reward.
% Compared to the Base model, it improved on all Basic Properties and Test Smells: $\uparrow$ 23.2\% Assertions, $\uparrow$ 17.9\% Focal calls, $\downarrow$ 2.22\% Duplicate Assertions, and $\downarrow$ 2.53\% Conditionals/Exceptions; however, it produced 6.1\% fewer tests with Descriptive names and 11.0\% fewer tests with Comments.
% This model also improved on all Basic Properties and Test Smells compared to the GPT-4 model: $\uparrow$ 15.3\% Assertions, $\uparrow$ 0.3\% Focal calls, $\downarrow$ 0.01\% Duplicate Asserts, and $\downarrow$ 2.48\% Conditionals/Exceptions.


%%%%% Original Combined Reward
% \noindent\textbf{Combined Reward:}
% Table \ref{tab:additive-reward} shows the results of Combined Reward training.
% % We optimized all combinations of two, three, or four properties.
% On 2-property optimization, 6/12 optimized properties improved and 6/12 regressed, compared to the corresponding Individual Reward settings.
% On 3-property optimization, 4/9 optimized properties improved while 5/9 regressed. Some properties regressed substantially, such as the Assert and Focal properties in the \ppomodel{(\goodmark{} Assert + \goodmark{} Focal + \badmark{} Conditional/Exception)} setting; we observed this can occur due to the policy model diverging from the starting weights in order to increase the modeled reward.
% The Assert property improved in almost all cases, while the Focal, Duplicate Assert, and Conditional/Exception properties regressed in more than half of the cases.
% % Properties Descriptive and Comments are withheld for space; we did not optimize them since they did not perform well on individual rewards.

% By comparing the results of 3-property configurations with 2-property configurations, we see that adding a third property to the reward model often did not cause the policy model to improve on that property. For example, comparing \ppomodel{(\goodmark{} Assert + \goodmark{} Focal)} with \ppomodel{(\goodmark{} Assert + \goodmark{} Focal + \badmark{} Duplicate assert)}, the latter model generated \textit{more} duplicate assertions than the former. The additional property may make the modeled reward more difficult to optimize, preventing the policy model from discovering an optimal policy. %\BENJAMIN{Why?}

% Similarly, optimizing All Properties in one reward model performed worse than some 2- or 3-property settings. This may be because the space of possible rewards is larger, ranging from -1 to 4, and thus the policy model was not able to sufficiently optimize its completions but got stuck in a local minimum which earned relatively high reward from the reward model. %\BENJAMIN{What measures could be taken to ameliorate this?}

% % \BENJAMIN{Can we make the case that the Combined approach works better in some cases than sequential, such as with unrelated properties?}

% % \BENJAMIN{For additive reward training: Observations from Table \ref{tab:additive-reward} (additive reward):
% % \begin{itemize}
% %     \item On 2-property, 6 optimized properties improved and 6 regressed compared to individual PPO.
% %     \item On 3-property, 4 optimized properties improved and 5 regressed.
% %     \item Properties Assert and Try or Conditional improved in the majority of cases.
% %     \item Properties Focal and Duplicate asserts regressed in the majority of cases.
% %     \item Properties Descriptive and Comments are withheld for space; we did not optimize them since they did not perform well on individual rewards.
% %     \item All Properties did not perform the best. \BENJAMIN{Why?}
% % \end{itemize}}

% % Next steps
% % For some properties, the last checkpoint (step 150) performed the best on the validation dataset; more training epochs may further improve the model.
% % Additive reward for all 4 properties will come soon. It requires adjusting our resampling strategy, similar to 2-property training.

% \BENJAMIN{Summarize in one sentence. Merge with the following paragraph but still make the point about synergy.}
% In the Combined Reward setting, two settings improved on all properties: \ppomodel{(\goodmark{} Assert + \badmark{} Conditional/Exception)} and \ppomodel{(\goodmark{} Focal + \badmark{} Duplicate assert + \badmark{} Conditional/Exception)}.
% Notably, the properties optimized by these models are not likely to be correlated or dependent (compared to e.g. Asserts and Duplicate Asserts, which are certainly interdependent), which may indicate that the Combined Reward setting works most effectively when there are fewer dependencies between properties.
% % \BENJAMIN{Further discussion?}
% % In the Combined Reward setting, the model \ppomodel{\goodmark{} Focal + \badmark{} Dupl. asserts + \badmark{} Try/Cond.} performed the best overall since it improved all three optimized properties.

% \BENJAMIN{Summarize in one sentence. Remove redundancy from RQ2.}
% Observing the best models trained with the Combined and Sequential Reward strategies, we see that RL-finetuned models consistently improved over the Base Codex. The highest-performing model overall was \ppomodel{(\goodmark{} Focal + \badmark{} Conditional/Exception)}, trained with Combined Reward.
% Compared to the Base model, it improved on all Basic Properties and Test Smells: $\uparrow$ 23.2\% Assertions, $\uparrow$ 17.9\% Focal calls, $\downarrow$ 2.22\% Duplicate Assertions, and $\downarrow$ 2.53\% Conditionals/Exceptions; however, it produced 6.1\% fewer tests with Descriptive names and 11.0\% fewer tests with Comments.
% %, since it generated the most positive properties and avoided the most test smells.
% This model also improved on all Basic Properties and Test Smells compared to the GPT-4 model: $\uparrow$ 15.3\% Assertions, $\uparrow$ 0.3\% Focal calls, $\downarrow$ 0.01\% Duplicate Asserts, and $\downarrow$ 2.48\% Conditionals/Exceptions.

% % \BENJAMIN{We can note that overall, most settings of RLSQM improve over SFT and Base models.}

% % \setlength\fboxsep{2pt}
% % \vspace{-0.05cm}
% % \begin{center}
% % \colorbox{gray!20}{
% % \begin{minipage}[t]{0.97\linewidth}
% % {\bf Summary for RQ$_3$.}
% % RL from Sequential and Combined Rewards (optimizing \ppomodel{\goodmark{} Focal + \badmark{} Conditional/Exception}) improved upon the Base model further than Individual Rewards by increasing best practices: up to $\uparrow$ 23.2\% Assertions and 
% % $\uparrow$ 17.9\% Focal calls, and reducing test smells: up to $\downarrow$ 2.22\% Duplicate Assertions and $\downarrow$ 2.53\% Conditionals/Exceptions.
% % \end{minipage}
% % }
% % \end{center}
% % \setlength\fboxsep{0pt}


